A Low-Subpacketization High-Performance MIMO Coded Caching Scheme

In this paper, we study how coded caching can be efficiently applied to multiple-input multiple-output (MIMO) communications. This is an extension to cache-aided multiple-input single-output (MISO) communications, where it is shown that with an $L$-antenna transmitter and coded caching gain $t$, a cumulative coded caching and spatial multiplexing gain of $t+L$ is achievable. We show that, interestingly, for MIMO setups with $G$-antenna receivers, a coded caching gain larger than MISO setups by a multiplicative factor of $G$ is possible, and the full coded caching and spatial multiplexing gain of $Gt+L$ is also achievable. Furthermore, we propose a novel algorithm for building low-subpacketization, high-performance MIMO coded caching schemes using a large class of existing MISO schemes.

==> ExtAbstract.tex <==




%In this paper, we extend the applicability of coded caching to \ac{MIMO} communications with multi-antenna receivers. We show that \ac{MIMO} coded caching can be considered as an extension of the shared-cache setting studied in~\cite{parrinello2019fundamental,parrinello2020extending}. In shared-cache setups, a number of single-antenna users are aided by a smaller number of shared-cache nodes (which can be, e.g., helper nodes) while requesting data from a multi-antenna transmitting server. To extend this model to \ac{MIMO} coded caching, we can assume each shared-cache node represents a multi-antenna receiver, and each single-antenna user is replaced by an antenna element. Such an extension paves the way to using the optimality results in~\cite{parrinello2019fundamental,parrinello2020extending} to \ac{MIMO} coded caching. Specifically, in case all the users in a \ac{MIMO} setup have more than $G$ number of receiving antennas\footnote{$G$ represents the number of independent streams transmitted to each receiver.}, assuming large enough $L$, we get the interesting result that the coded caching gain $t$ can be multiplied by $G$, and a cumulative single-shot \ac{DoF} of $Gt+L$ becomes achievable.

%We also propose a new algorithm for creating \ac{MIMO} coded caching schemes, where we elevate baseline linear \ac{MISO} schemes already available in the literature to be applicable to \ac{MIMO} setups while achieving the increased \ac{DoF} of $Gt+L$. The elevation method is applicable when the number of dedicated streams to each receiver divides the number of transmit antennas (i.e., when $\eta := \frac{L}{G}$ is an integer), and achieves the full \ac{DoF} of $Gt+L$ if the baseline \ac{MISO} scheme supports the \ac{DoF} of $t+L$. This enables designing low-complexity, low-subpacketization \ac{MIMO} schemes with full \ac{DoF} using an appropriate \ac{MISO} scheme such as the one in~\cite{salehi2020lowcomplexity}.
%
%We show that in such a scenario, the coded caching gain can be increased interestingly by a multiplicative factor proportional to the receiver antenna count. In other words, if every user has $G$ receiving antennas and $\frac{L}{G}$ is an integer, we propose a novel coded caching scheme where with every single transmission, it is possible to send $Gt + L$ independent streams to the users. 
%
%The key to achieving this multiplicative improvement in caching gain is in the use of signal-level interference cancellation approach similar to the one presented in~\cite{lampiris2018adding}, as well as a shared-cache user grouping mechanism similar to that presented in~\cite{salehi2020lowcomplexity} for enabling extremely low subpacketization requirement. In this extended abstract, we introduce the general procedure and clarify the idea with a small example. A more detailed explanation will be provided in the extended version of the paper. To the best of our knowledge, this work is the first one to present the possibility of such an improved \ac{DoF} gain in cache-aided \ac{MIMO} communications.
%
%In a nutshell, the elevation algorithm works as follows: for a given $K$-user \ac{MIMO} network with $L$ antennas at the transmitter and more than $G$ antennas at each receiver, %\footnote{In fact, $L$ and $G$ represent the maximum number of independent streams at the transmitter and receivers, respectively. For simplicity, here we assume the number of independent streams is equal to the number of antennas, i.e., the channel matrix from the transmitter to each receiver is full-rank. Moreover, we also assume the RX processing is antenna-specific (i.e. no beamforming is done at the receiver side).} 
%we first consider a virtual \ac{MISO} network with the same number of $K$ users and caching gain $t$, but with $\eta$ antennas at the transmitter. Then, we design cache placement and transmission vectors for the virtual network following one of the available linear \ac{MISO} schemes in the literature (the baseline scheme should support signal-level interference cancellation as explained later on). Finally, cache contents for users in the real network are set to be the same as in the virtual network, and the transmission vectors are \textit{stretched} to support multi-antenna receivers and increased \ac{DoF}. In this extended abstract, we clarify the procedure using an example, and leave the detailed explanation for the extended version of the paper. %For clarification, here we review these three steps for a small, example network.

%Before proceeding with the example, let us define some notations. For any integer $J$, we use $[J]$ to denote the set of numbers $\{1,2,...,J\}$. The set of users is shown by $\CK$. A general file in the library is shown by $W$, and the file requested by user $u_k \in \CK$ is denoted by $W(k)$. Zero-forcing transmit beamformer vectors for real and virtual networks are denoted by $\Bw_{\CR}$ and $\hat{\Bw}_{\CR}$, respectively, where the set $\CR$ includes the indices of the user specific streams at which the data is nulled-out by the beamformer. For notation simplicity, we remove the brackets while explicitly writing the stream indices in $\CR$. We also use $\Sfs_k^g$, $g \in [G]$, to refer to stream $g$ intended for user $u_k$. %Finally, the bit-wise XOR operation is denoted by $\oplus$.
%Finally, for two sets $\CA$ and $\CB$, $\CA \backslash \CB$ denotes the set of elements in $\CA$ that are not in $\CB$.

Now, assume a small network with $K=6$ users and caching gain $t=1$, where the transmitter has $L=4$ and every receiver has two antennas.
% at the transmitter, and $G=2$ antennas at each receiver. 
%The coded caching gain is given as $t=1$. 
Using \ac{MISO} schemes, the maximum achievable \ac{DoF} for this network is $L+t = 5$ (multiple receive antennas can be used for additional beamforming gain). However, with the proposed elevation algorithm, the \ac{DoF} value can be increased to $Gt+L=6$, assuming $G=2$ parallel streams for each user are supportable by the channel conditions. Without loss of generality, let us assume the reduced-subpacketization scheme in~\cite{salehi2020lowcomplexity} is chosen as the baseline \ac{MISO} scheme.
%
%Using the original coded caching scheme in~\cite{shariatpanahi2018physical}, the maximum achievable \ac{DoF} for this network would be $L+t = 5$. Note that with this scheme, multiple antennas at the receivers are used only to improve the \ac{SINR}. However, we show that with the new scheme, it is possible to serve $Gt+L =6$ independent data streams with every single transmission (i.e., the achievable \ac{DoF} is increased to 6). 
The first step is to find proper parameters for the virtual \ac{MISO} network. Clearly, the virtual network has the same number of $K=6$ users and caching gain $t=1$, but with $\eta = 2$ antennas at the transmitter and one antenna at each receiver. Cache placement in the virtual network directly follows that of~\cite{salehi2020lowcomplexity}, i.e., every file $W$ is first split into $K=6$ equal-sized \textit{packets} denoted by $W_p$, $p \in [6]$, and then, each packet is split into $t+\eta=3$ smaller \textit{subpackets} denoted by $W_p^q$, $q \in [3]$. Finally, in the cache memory of user $u_k$, we store $W_k^q$, for every $W$ and $q$. 

%For simplicity, we use the tabular view in Figure~\ref{fig:Graphical_base} to represent the cache placement in this network. In this representation, a darkly shaded cell in row $p$ and column $k$ denotes that the file parts $W_p^q$ for every $W$, $q$ are stored in the cache memory of user $u_k$.

%\input{Figs/GraphicalBase}
\input{Figs/Trans_comp_virtual}

For notational simplicity, let us assume $W(1) \equiv A$, $W(2) \equiv B$, ..., and $W(6) \equiv F$ (note that it is possible for some users to request the same file). Using the coded caching scheme in~\cite{salehi2020lowcomplexity} for the virtual network, the first and second transmission vectors (corresponding to the transmissions in the first and second time intervals) are built as\footnote{Note that virtual beamformer vectors $\hat{\Bw}_{\CR}$ are defined only to clarify the transmission (and decoding) process in the virtual network. We do not need to calculate them at any step.}
\begin{equation}
\label{eq:trans_vector_exmp_virtual}
\begin{aligned}
    \hat{\Bx}_1 &= A_2^1 \hat{\Bw}_3 + B_1^1 \hat{\Bw}_3 + C_1^1 \hat{\Bw}_2 , \\
    \hat{\Bx}_2 &= A_3^1 \hat{\Bw}_4 + C_1^2 \hat{\Bw}_4 + D_1^1 \hat{\Bw}_3 .
\end{aligned}
\end{equation}
%where $\Bx_1$ and $\Bx_2$ deliver parts of the requested data to user sets $\{u_1,u_2,u_3\}$ and $\{u_1,u_3,u_4\}$, respectively.
For better clarification, a graphical representation for $\hat{\Bx}_1$ and $\hat{\Bx}_2$ is provided in Figure~\ref{fig:subhatnoxor}. This representation follows the same principles as in~\cite{salehi2020lowcomplexity}, i.e., 
%
%Following the same representation as in~\cite{salehi2020lowcomplexity}, a graphical view of $\Bx_1$ and $\Bx_2$ are shown in Figure~\ref{fig:subhatnoxor}. In graphical representations, 
a black cell means (every subpacket of) the respective data part is available in the cache memory, and a gray cell indicates that (a subpacket of) the respective part is sent during the transmission. 


%Without loss of generality, let us consider the decoding process for $\Bx_1$. As we have used zero-forcing beamformers, after this transmission, users $u_1$, $u_2$ and $u_3$ receive
%\begin{equation}
%    \begin{aligned}
%        y_1(1) &= A_2^1 \Bh_1^H \Bw_3 + B_1^1 \Bh_1^H \Bw_3 + C_1^1 \Bh_1^H \Bw_2 + z_1(1) , \\
%        y_1(2) &= A_2^1 \Bh_2^H \Bw_3 + B_1^1 \Bh_2^H \Bw_3 + z_1(2) , \\
%        y_1(3) &= C_1^1 \Bh_3^H \Bw_2 + z_1(3) , \\
        %y_2(1) &= (A_2^2 \oplus B_1^2) \Bh_1^H \Bw_3 + (A_4^1 \oplus D_1^1) \Bh_1^H \Bw_2 + z_2(1) , \\
%    \end{aligned}
%\end{equation}
%where $\Bh_k$ denotes the (virtual) channel vector for $u_k$,\footnote{The channel vectors here are defined only to explain the decoding process with the signal-level interference cancellation approach within the virtual \ac{MISO} network. They do not have a physical interpretation.} and $z_1(k)$ represents the \ac{AWGN} at the receiver of $u_k$ during the transmission of $\Bx_1$.
%With $y_1(1)$ at its receiver, user $u_1$ first reconstructs $B_1^1 \Bh_1^H \Bw_3$ and $C_1^1 \Bh_1^H \Bw_2$ using its cache contents\footnote{We assume the equivalent channels $\Bh_1^H \Bw_3$ and $\Bh_1^H \Bw_2$ can be (ideally) estimated from the stream specific demodulation pilots [REF].} and removes them from $y_1(1)$, and then, decodes $A_2^1$ interference-free. Similarly, users $u_2$ and $u_3$ also remove the remaining interference using their cache contents and decode (parts of) their requested data interference-free.
%As the remaining interference is here removed with the help of cache contents \textit{before} decoding data, we call this approach \textit{signal-level} interference cancellation. In contrast, in the \textit{bit-level} approach, the interference is removed \textit{after} the decoding is completed. A good example of the bit-level approach can be found in the original \ac{MISO} scheme in~\cite{shariatpanahi2018physical}, where the cache-aided interference removal (with XOR operation) is done after decoding the codewords.\footnote{It should be noted that the bit-level approach in~\cite{shariatpanahi2018physical} can be easily transformed to the signal-level approach by avoiding the XOR operation inside codewords and using a separate beamformer vector for each data packet. As a result, the proposed elevation scheme can also be applied to the coded caching scheme in~\cite{shariatpanahi2018physical}, but with an additional step. This is explained in more detail in the extended version of the paper.}

%first decodes $(A_2^1 \oplus B_1^1)$ and $(A_3^1 \oplus C_1^1)$ using a \ac{SIC} receiver, and then uses its cache contents to remove $B_1^1$ and $C_1^1$ to get $A_2^1$ and $A_3^1$ interference-free. As the cache contents are used after the decoding process, this procedure is called the bit-level interference cancellation approach. 
%From a different perspective, we can built this transmission vector as
%\begin{equation}
%\begin{aligned}
%\label{eq:trans_vector_exmp_signal_level_virtual}
%    \Bar{\Bx}_1 = A_2^1 \Bw_3 + B_1^1 \Bar{\Bw}_3 + A_3^1 \Bw_2 + C_1^1 \Bar{\Bw}_2 + B_3^1 \Bw_1 + C_2^1 \Bar{\Bw_1},
%\end{aligned}
%\end{equation}
%where the bars are used only to distinguish various beamforming vectors that zero-force data at the same subset of users. With this approach, $u_1$ receives
%\begin{equation}
%\begin{aligned}
%    \Bar{y}_1(1) = &A_2^1 \Bh_1^H \Bw_3 + B_1^1 \Bh_1^H \Bar{\Bw}_3 \\
%    &+ A_3^1 \Bh_1^H \Bw_2 + C_1^1 \Bh_1^H \Bar{\Bw_2} + z_1(1) ,
%\end{aligned}
%\end{equation}
%and has to reconstruct and remove the interference terms $B_1^1 \Bh_1^H \Bar{\Bw}_3$ and $C_1^1 \Bh_1^H \Bar{\Bw}_2$ using its cache contents, before using a \ac{SIC} receiver (for getting $A_2^1$ and $A_3^1$ interference-free). As the interference is now removed before decoding the received signal, this approach is called signal-level interference cancellation. 

%Note that using the same signal-level approach, without any \ac{DoF} loss, we can also use the following two transmissions instead of $\Bar{\Bx}_1$ to avoid the SIC receiver
%\begin{equation}
%\begin{aligned}
%\label{eq:trans_vector_exmp_signal_level_virtual_decouple}
%    \Bar{\Bx}^1_1 &= A_2^1 \Bw_3 + B_1^1 \Bar{\Bw}_3 + C_1^1 \Bar{\Bw}_2  \\
%    \Bar{\Bx}^2_1 &= A_3^1 \Bw_2 + B_3^1 \Bw_1 + C_2^1 \Bar{\Bw}_1.
%\end{aligned}
%\end{equation}
%In other words, without any \ac{DoF} loss, we can use more transmissions to avoid \ac{SIC} receivers (this approach is similar to controlling the multiple access channel size with the $\beta$ parameter in~\cite{tolli2017multi}). In this paper, for its simplicity, we use this model to explain our new scheme for the increased \ac{DoF} (note that it is also possible to use the \ac{SIC}-requiring approach as in~\eqref{eq:trans_vector_exmp_signal_level_virtual}, and this selection is only made to make the explanation simpler). 

%Moreover, we also use a simple graphical representation to show how various transmission vectors are formed. In Figure~\ref{fig:Graphical_base}, we have provided the graphical representation for both bit- and signal-level transmission vectors $\Bx_1$ and $\Bar{\Bx}_1$, as presented in~\eqref{eq:trans_vector_exmp_bit_level} and~\eqref{eq:trans_vector_exmp_signal_level_virtual}, respectively. In this figure, darkly shaded cells represent cached data parts at different users, while lightly shaded ones denote the parts being transmitted with the transmission vectors. Similarly, in Figure~\ref{fig:subhatnoxor}, we have provided the graphical representation for \ac{SIC}-avoiding signal-level transmission vectors $\Bar{\Bx}_1^1$ and $\Bar{\Bx}_1^2$ as presented in~\eqref{eq:trans_vector_exmp_signal_level_virtual_decouple}.


%The graphical representation for these two approaches is provided in Figure~\ref{fig:subhatnoxor}, where the lightly shaded cells represent the file parts being sent during each transmission.

%\input{Figs/GraphicalBase}

Now, transmission vectors for the original \ac{MIMO} setup can be found by stretching the transmission vectors in~\eqref{eq:trans_vector_exmp_virtual}. For stretching, for every term $W_p^q(k) \hat{\Bw}_{\CR}$ in a transmission vector of the virtual network, we 
%
%Using the decoupled version as in~\eqref{eq:trans_vector_exmp_signal_level_virtual_decouple} for the virtual network, we can \textit{elevate} the transmission vectors to support the extended \ac{DoF} in the original network. 
%
%The procedure is as follows: 
first split $W_p^q(k)$ into $G$ smaller parts $W_p^{q,g} (k)$, $g \in [G]$, and then replace the whole term with
\begin{equation}
    W_p^q(k) \hat{\Bw}_{\CR} \; \rightarrow \; W_p^{q,1} (k) \Bw_{\CR_1} +  ... + W_p^{q,G} (k) \Bw_{\CR_G} ,
\end{equation}
where the new zero-forcing sets $\CR_g$ are built as
\begin{equation}
    \CR_g = \bigcup_{u_{\Bar{k}} \in \CR} \{ \Sfs_{\Bar{k}}^1, ... , \Sfs_{\Bar{k}}^G \} \; \cup \; \{ \Sfs_k^1, ... , \Sfs_k^G \} \backslash \{ \Sfs_k^g \} .
\end{equation}
In other words, instead of a data stream $W_p^q(k)$ for user $u_k$, we consider $G$ parallel streams $W_p^{q,g}(k)$, where each stream will be assigned distinct receive beamformer at user $u_k$. Moreover, if the zero-forcing set for $W_p^q (k)$ is $\CR$, the zero-forcing set for $W_p^{q,g}(k)$ includes every dedicated stream for every user in $\CR$, as well as $G-1$ streams for $u_k$ (i.e., every stream for $u_k$ except $\Sfs_k^g$). This means $W_p^{q,g}(k)$ must be zero-forced at a total number of
\begin{equation}
    (\eta-1)G + G-1 = \eta G -1 = L-1 
\end{equation}
locations (i.e, streams), which is indeed possible as we have $L$ antennas at the transmitter. For the example network, the stretched version of $\hat{\Bx}_1$ can be written as
\begin{equation}
\begin{aligned}
    {\Bx}_1 =& A_2^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + A_2^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} \\
    & + B_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
    & + C_1^{1,1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1} ,
\end{aligned}
\end{equation}
and for $\hat{\Bx}_2$ we can write
\begin{equation}
\begin{aligned}
    {\Bx}_2 =& A_3^{1,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^2} + A_3^{1,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_1^1} \\
    & + C_1^{2,1} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^2} + C_1^{2,2} \Bw_{\Sfs_4^1,\Sfs_4^2,\Sfs_3^1} \\
    & + D_1^{1,1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^2} + D_1^{1,2} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_4^1} .
\end{aligned}
\end{equation}
Note that in this example, zero-forcing at three locations is possible as the number of transmitter antennas is given as $L=4$. The graphical representations for these transmissions are provided in Figures~\ref{fig:extended} and~\ref{fig:extended_second}. As can be seen, they seem like the stretched versions of the base representations provided in Figure~\ref{fig:subhatnoxor}, and hence, we use the term \textit{stretching} to denote the proposed set of operations.

\input{Figs/Trans_extended_first_trans}

\input{Figs/Trans_extended_second}

For clarification, let us review the decoding process for each stream of user $u_1$ in ${\Bx}_1$. As we have used zero-forcing beamformers, the received signal vector at user $u_1$ is 
\begin{equation}
    \begin{aligned}
        \By_1 = \BH_1 {\Bx}_1 + \Bz_1=& A_2^{1,1} \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + \BI_1 +  \Bz_1 ,
    \end{aligned}
\end{equation}
where $\BH_{1} \in \mathbb{C}^{2 \times 4}$ denotes the channel matrix between user $1$ and the transmitter, $\Bz_1$ represents the \ac{AWGN} vector at $u_1$ during the transmission of $\Bx_1$, and $\BI_1$ denotes the interference term. Now, the stream-specific received signal for $\Sfs_1^1$ can be written as
\begin{equation}
    \begin{aligned}
        y_1(\Sfs_1^1) := \Bu_{\Sfs_1^1}^H \By_1 =& A_2^{1,1} \Bu_{\Sfs_1^1}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^2} + I_1(\Sfs_1^1) +  z_1(\Sfs_1^1) ,
    \end{aligned}
\end{equation}
where $\Bu_{\Sfs_1^1} \in \mathbb{C}^{2}$ denotes the dedicated receive beamformer for stream $\Sfs_1^1$ at user $1$ and $z_1(\Sfs_1^1)$ represents its corresponding noise. The interference term $I_1(\Sfs_1^1)$ is defined as
\begin{equation}
    \begin{aligned}
        I_1(\Sfs_1^1) := & + B_1^{1,1} \Bu_{\Sfs_1^1}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
        & + C_1^{1,1} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bu_{\Sfs_1^1}^H \BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1}.
    \end{aligned}
\end{equation}
However, the user $u_1$ has $B_1^1$ and $C_1^1$ in its cache memory, and hence, it can reconstruct and remove the whole interference term $I_1(\Sfs_1^1)$ from $y_1(\Sfs_1^1)$,\footnote{We assume the term ($\Bu_{\Sfs^{g}_{{k}}}^{H} \BH_{k} \Bw_{\CR}$) can be estimated from stream-specific demodulation pilots.} to decode $A_2^{1,1}$ interference-free. Similarly, the stream-spicific received signal for $\Sfs_1^2$ of user $u_1$ is
\begin{equation}
    \begin{aligned}
        y_1(\Sfs_1^2) :=\Bu_{\Sfs_1^2}^H \By_1 =& A_2^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_1^1} + I_1(\Sfs_1^2) +  z_1(\Sfs_1^2) ,
    \end{aligned}
\end{equation}
where $\Bu_{\Sfs_1^2} \in \mathbb{C}^{2}$ denotes the dedicated receive beamformer for stream $\Sfs_1^2$ at user $1$ and the interference term $I_1(\Sfs_1^2)$ is defined as
\begin{equation}
    \begin{aligned}
        I_1(\Sfs_1^2) := & + B_1^{1,1} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^2} + B_1^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_3^1,\Sfs_3^2,\Sfs_2^1} \\
        & + C_1^{1,1} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^2} + C_1^{1,2} \Bu_{\Sfs_1^2}^H\BH_{1} \Bw_{\Sfs_2^1,\Sfs_2^2,\Sfs_3^1}.
    \end{aligned}
\end{equation}
Again, the user $u_1$ can reconstruct and remove the interference term $I_1(\Sfs_1^2)$ using its cache contents, and decode $A_2^{1,2}$ interference-free. Following the same procedure for users $u_2$ and $u_3$, each of them can decode two parallel streams after the transmission of $\Bx_1$, and hence, the increased \ac{DoF} value of $6$ can be achieved for the considered \ac{MIMO} setup. It should be noted that, as the remaining interference is here removed with the help of cache contents \textit{before} decoding data, we call this approach \textit{signal-level} interference cancellation. In contrast, in the \textit{bit-level} approach, the interference is removed \textit{after} the decoding is completed. A good example of the bit-level approach can be found in the original \ac{MISO} scheme in~\cite{shariatpanahi2018physical}, where the cache-aided interference removal (with XOR operation) is done after decoding the codewords. However, the bit-level approach in~\cite{shariatpanahi2018physical} can be easily transformed to the signal-level approach by avoiding the XOR operation inside codewords and using a separate beamformer vector for each data packet. As a result, the proposed elevation algorithm can also be applied to the coded caching scheme in~\cite{shariatpanahi2018physical}, but with an additional step. This is explained in more detail in the extended version of the paper.

In summary, our new scheme enables $t+\eta$ users to be served with each transmission, and delivers $G$ independent streams to each of these users. This results in a total number of $G(t+\eta) = Gt+L$ independent streams, and hence, a multiplication in the coded caching gain $t$ compared to the state-of-art. %To the best of our knowledge, this is the first scheme to show such a multiplicative increase in the coded caching gain is possible in cache-enabled \ac{MIMO} setups.
If the baseline \ac{MISO} scheme is chosen as the one in~\cite{salehi2020lowcomplexity},
the total subpacketization requirement for the elevated \ac{MIMO} scheme is
\begin{equation}
    G K (t + \eta) = K(Gt + L)
    %G \binom{K}{t} \binom{K-t-1}{\eta - 1}.
\end{equation}
In the extended version of this paper, we present a detailed explanation of the proposed method, and thoroughly investigate the possibility of using other baseline \ac{MISO} schemes. We also relax the antenna-specific RX processing assumption by considering stream-specific processing, and compare our algorithm with the state-of-art from the achievable \ac{DoF} and subpacketization requirement perspectives.
%A detailed explanation of the proposed method, the possibility of using other baseline \ac{MISO} schemes, and more comparisons with the state-of-art from the achievable \ac{DoF} and subpacketization requirement perspectives are due for the extended version of this paper.

%The text needs a major revision:
%\begin{enumerate}
%    \item The literature review part should be updated to include works by Petros and Emanuele on shared cache settings~\cite{parrinello2019fundamental,parrinello2020extending}.
%    \item Our contribution should be clarified: we consider a MIMO system and based on the previous results from Emanuele and Petros, show that multiple receiving antennas boost the coded caching gain with a multiplicative factor.
%    \item Then, we provide a simple extension scheme, that can be applied to any based MISO scheme, which achieves the full enhanced coded caching gain in the MIMO setup.
%    \item We show that by using this extension on top of the base scheme in the TWC work, we can have a linear (or quadratic) subpacketization increase while achieving the full enhanced caching gain.
%    \item The example should be updated accordingly; it should reflect transmission vectors built with the TWC scheme instead of MS.
%\end{enumerate}

==> Figs/GraphicalBase.tex <==
\begin{figure}[ht]
    \centering
        \centering
        \begin{tikzpicture}[scale = 0.57]
            % grid
            \begin{scope}<+->;
            \draw[step=1cm,thick,black!90] (1,0) grid (7,6);
            \draw[thin,black!70](0,0)to(1,0);
            \draw[thin,black!70](0,1)to(1,1);
            \draw[thin,black!70](0,2)to(1,2);
            \draw[thin,black!70](0,3)to(1,3);
            \draw[thin,black!70](0,4)to(1,4);
            \draw[thin,black!70](0,5)to(1,5);
            \draw[thin,black!70](0,6)to(1,6);
            \draw[thin,black!70](1,6)to(1,7);
            \draw[thin,black!70](2,6)to(2,7);
            \draw[thin,black!70](3,6)to(3,7);
            \draw[thin,black!70](4,6)to(4,7);
            \draw[thin,black!70](5,6)to(5,7);
            \draw[thin,black!70](6,6)to(6,7);
            \draw[thin,black!70](7,6)to(7,7);
            %\draw[pattern=crosshatch, pattern color=black!30](4,0)rectangle(5,5);
            %\draw[very thick](1,0)to(1,4)to(3,4)to(3,0);
            %\draw[very thick](1,6)to(1,5)to(3,5)to(3,6);
            %\draw[very thick](0,4)to(1,4)to(1,5)to(0,5);
            %\draw[very thick](6,4)to(3,4)to(3,5)to(6,5);
            \end{scope}
            % function
            \begin{scope}
            \FillHatch{7}{1}{2};
            \FillHatch{7}{1}{3};
            \FillHatch{7}{1}{4};
            \FillHatch{7}{2}{2};
            \FillHatch{7}{2}{3};
            \FillHatch{7}{2}{4};
            \FillHatch{7}{3}{2};
            \FillHatch{7}{3}{3};
            \FillHatch{7}{3}{4};
            \FillHatch{7}{4}{2};
            \FillHatch{7}{4}{3};
            \FillHatch{7}{4}{4};
            \FillHatch{7}{2}{1};
            \FillHatch{7}{3}{1};
            \FillHatch{7}{4}{1};
            
            \FillBlack{7}{2}{2};
            \FillBlack{7}{3}{3};
            \FillBlack{7}{4}{4};
            \FillBlack{7}{5}{5};
            \FillBlack{7}{6}{6};
            \FillBlack{7}{7}{7};
            
            \FillGray{7}{2}{3};
            \FillGray{7}{2}{4};
            \FillGray{7}{3}{2};
            \FillGray{7}{3}{4};
            \FillGray{7}{4}{2};
            \FillGray{7}{4}{3};
            
            \PutText{7}{2}{1}{$W_1^q$};
            \PutText{7}{3}{1}{$W_2^q$};
            \PutText{7}{4}{1}{$W_3^q$};
            \PutText{7}{5}{1}{$W_4^q$};
            \PutText{7}{6}{1}{$W_5^q$};
            \PutText{7}{7}{1}{$W_6^q$};
            \PutText{7}{1}{2}{$u_1$};
            \PutText{7}{1}{3}{$u_2$};
            \PutText{7}{1}{4}{$u_3$};
            \PutText{7}{1}{5}{$u_4$};
            \PutText{7}{1}{6}{$u_5$};
            \PutText{7}{1}{7}{$u_6$};
            \end{scope}
        \end{tikzpicture}
    \caption{Graphical representation for bit-level and \ac{SIC}-requiring signal-level transmissions $\Bx_1$ and $\Bar{\Bx}_1$}
    \label{fig:Graphical_base}
\end{figure}
